ContraCLM: Contrastive Learning For Causal Language Model

Despite exciting progress in causal language models, the expressiveness of the representations is largely limited due to poor discrimination ability. To remedy this issue, we present ContraCLM, a novel contrastive learning framework at both token-level and sequence-level. We assess ContraCLM on a variety of downstream tasks. We show that ContraCLM enhances discrimination of the representations and bridges the gap with the encoder-only models, which makes causal language models better suited for tasks beyond language generation. Specifically, we attain $44\%$ relative improvement on the Semantic Textual Similarity tasks and $34\%$ on Code-to-Code Search tasks. Furthermore, by improving the expressiveness of the representations, ContraCLM also boosts the source code generation capability with $9\%$ relative improvement on execution accuracy on the HumanEval benchmark.

==> tables/main/code_search_and_completion.tex <==
\begin{table*}[t]
    % \setlength{\tabcolsep}{5pt}
    \begin{center}
    {\normalsize{
        \resizebox{\linewidth}{!} {%
        \def\arraystretch{1.0}%
        \begin{tabular}{r c c c c c c c c}
        \toprule
        \multirow{3}{*}{Model} & \multicolumn{4}{c}{Text-to-Code Search}  & \multicolumn{4}{c}{Code Completion and Re-ranking} \\
        \cmidrule(lr){2-5} 
        \cmidrule(lr){6-9} 
        & \multirow{2}{*}{CoSQA} & \multirow{2}{*}{AdvTest} & \multirow{2}{*}{CSN} & \multirow{2}{*}{Avg.} & \multicolumn{2}{c}{Pass@k} & \multicolumn{2}{c}{Ranked Pass@k} \\
        \cmidrule(lr){6-7} 
        \cmidrule(lr){8-9}
        & & & & & k=1 & k=5 & k=1 & k=5 \\ 
        \midrule
        CodeGen         &  8.39 & 1.65 & 3.88 & 4.64 & 12.65 & 16.89 & 13.42 \textsubscript{(+0.77)} & 17.07 \textsubscript{(+0.18)} \\ 
        \midrule
        CLM             &  11.03 & 2.51 & 5.67 & 6.40 & 13.42 & 18.08 & 15.38 \textsubscript{(+1.96)} & 18.29 \textsubscript{(+0.21)} \\
        \midrule
        SimCTG          &  10.80 & \textbf{3.81} & 8.33 & 7.65 & 13.26 & 17.29 & 15.24 \textsubscript{(+1.98)} & 18.29 \textsubscript{\textbf{(+1.00)}} \\
        \midrule
        \ourmethodtok         &  10.71 & 3.73 & \textbf{8.69} & \textbf{7.71} & 12.96 & 17.01 & 15.24 \textsubscript{(+2.96)} & 17.68 \textsubscript{(+0.67)} \\
        \hdashline\noalign{\vskip 0.5ex}
        \ourmethodseq         &  9.96 & 3.03 & 6.21 & 6.40 & 13.64 & 15.85 & 16.99 \textsubscript{\textbf{(+3.35)}} & 16.46 \textsubscript{(+0.61)} \\
        \hdashline\noalign{\vskip 0.5ex}
        \ourmethod             &  \textbf{11.09} & 3.53 & 7.96 & 7.53 & \textbf{14.63} & \textbf{18.83} & \textbf{17.07} \textsubscript{(+2.44)} & \textbf{18.90} \textsubscript{(+0.07)} \\
        \bottomrule
        \end{tabular}
        }
    }}
    \caption{
    Evaluation results on text-to-code search, code completion, and re-ranking tasks.
    For code search, we report MRR score (\%), while for code completion and re-ranking, we report pass@k and ranked pass@k (the numbers in the subscript indicates the difference between ranked pass@k and pass@k). While \ourmethodtok outperforms the baselines on code search tasks, \ourmethod significantly outperforms the baselines in code completion and re-ranking tasks.
    }
    \label{tab:code_search_completion}
    \end{center}
\end{table*}



==> tables/main/text_to_code_main.tex <==
\begin{table*}[htbp]
    \begin{center}
    {\normalsize{
        % \resizebox{\linewidth}{!} {%
        \def\arraystretch{1.0}%
        \begin{tabular}{r c c c c}
        \toprule
        Model & CoSQA & AdvTest & CSN & Avg. \\ 
        \midrule
        CodeGen         &  8.39 & 1.65 & 3.88 & 4.64 \\ 
        \midrule
        CLM             &  11.03 & 2.51 & 5.67 & 6.40 \\
        \midrule
        SimCTG          &  10.80 & \textbf{3.81} & 8.33 & 7.65 \\
        \midrule
        \ourmethodtok         &  10.71 & 3.73 & \textbf{8.69} & \textbf{7.71} \\
        \hdashline\noalign{\vskip 0.5ex}
        \ourmethodseq         &  9.96 & 3.03 & 6.21 & 6.40 \\
        \hdashline\noalign{\vskip 0.5ex}
        \ourmethod             &  \textbf{11.09} & 3.53 & 7.96 & 7.53 \\
        \bottomrule
        \end{tabular}
        % }
    }}
    \caption{
    MRR score (\%) of zero-shot setting on text-to-code search task.
    }
    \label{tab:text_to_code}
    \end{center}
\end{table*}
